Managing LTL properties in Event-B refinement

Refinement in Event-B supports the development of systems via proof based step-wise refinement of events. This refinement approach ensures safety properties are preserved, but additional reasoning is required in order to establish liveness and fairness properties. In this paper we present results which allow a closer integration of two formal methods, Event-B and linear temporal logic. In particular we show how a class of temporal logic properties can carry through a refinement chain of machines. Refinement steps can include introduction of new events, event renaming and event splitting. We also identify a general liveness property that holds for the events of the initial system of a refinement chain. The approach will aid developers in enabling them to verify linear temporal logic properties at early stages of a development, knowing they will be preserved at later stages. We illustrate the results via a simple case study.

==> sec_conclusions.tex <==
%sec conclusion
%\begin{itemize}
%\item
%rigorously demonstrated how LTL properties hold in a development where all the new events will eventually be convergent
%\item
%provides theorems that provide this foundation
%\item 
%demonstrated that the application of the theory is already supported by the tools without change to the tools.
%\item
%insights gained thought beta dependent, so when beta-dependent, likely when the thing is convernget then can introduce the property
%\item
%
%%point about making something abstract at the beginning to give more motivation to the results of G(O_0)
%
%\end{itemize}

The paper has provided foundational results that justify when temporal properties hold at the end of a refinement chain for developments that contain anticipated, convergent and ordinary events, which goes beyond that presented in~\cite{B-LTL-Groslambert}.  The paper has also provided restrictions on the temporal properties in terms of being $\beta$-dependent which help to determine when a temporal property of interest should be introduced into the development chain.

